Design of Distributed Reconfigurable Robotics Systems with ReconROS

Robotics applications process large amounts of data in real-time and require compute platforms that provide high performance and energy-efficiency. FPGAs are well-suited for many of these applications, but there is a reluctance in the robotics community to use hardware acceleration due to increased design complexity and a lack of consistent programming models across the software/hardware boundary. In this paper we present ReconROS, a framework that integrates the widely-used robot operating system (ROS) with ReconOS, which features multithreaded programming of hardware and software threads for reconfigurable computers. This unique combination gives ROS 2 developers the flexibility to transparently accelerate parts of their robotics applications in hardware. We elaborate on the architecture and the design flow for ReconROS and report on a set of experiments that underline the feasibility and flexibility of our approach.

==> __latexindent_temp.tex <==
\section{Introduction}
\label{sec:Introduction}




Robotics systems are often distributed and can involve challenging computational tasks. Resource-efficiency is a fundamental challenge of such systems since large amounts of data must be processed with soft or even hard real-time constraints~\cite{Yanmaz+18}. Compared to implementations on CPUs and GPUs, FPGAs have been shown to offer higher performance and higher energy-efficiency for many of the involved tasks, e.g., for vision kernels~\cite{8782524}, for morphological image processing functions~\cite{7298356}, for feature detection and description algorithms~\cite{7577310}, and for convolutional neural network inference~\cite{8401525}. However, despite the demonstrated advantages of FPGAs, their uptake into the robotics domain is still limited for several reasons. On one hand, FPGA design and, all the more, software/hardware co-design are arguably more challenging than embedded software development. On the other hand, robotics engineers and application developers are typically not trained in FPGA circuit or hardware/software co-design.

High level synthesis (HLS) tools are available today that accept standard C/C++ for describing behavior and (semi-)automatically translate such descriptions to FPGA hardware. Although HLS tools increase productivity and are thus highly useful, a consistent programming model for implementing software and hardware functions is still lacking. Porting a robotics application from software to hardware or accelerating parts of the application in hardware requires the creation of suitable interfaces between software and FPGA hardware and very often leads to a re-development of substantial parts of the application.

Besides the demand for increased computational capacity and robustness, also the distributedness of typical robotics systems caused by the functional decomposition of larger applications into distinct processes that run in parallel, and often under real-time constraints, as well as the potential spatial distribution of these processes pose opportunities and challenges for hardware acceleration. 
There have been approaches for including reconfigurable hardware into distributed embedded systems, for example ReCoNets~\cite{reconet}, LMGS~\cite{lmgs} or RSS~\cite{rss}, but these approaches are not compatible with existing and widely-used software abstractions for creating distributed robotics systems.
 
In our work, we take up a very popular programming environment in the robotics domain, the robot operating system (ROS). ROS is a middleware layer that models applications as set of communicating nodes and provides several communication mechanisms for information exchange. 

In this paper, which is an extension of our previous conference publication~\cite{LP20}, we present the open source project {\sc ReconROS} as a novel integration of ROS with ReconOS~\cite{6636314}. This paper extends the conference publication mainly by more detailed explanations of the design flow and tool chain, by supporting also the ROS 2 communication paradigms actions and services, and by presenting and quantitatively evaluating {\sc ReconROS} on more advanced robotics applications, especially a distributed real-world mechatronics model with multiple FPGAs.
ReconOS provides an architecture and programming model to enable shared memory multi-threading for software and hardware threads. As a result, {\sc ReconROS} allows robotics developers to utilize hardware acceleration for ROS applications either as hardware-accelerated ROS nodes or as ROS nodes mapped completely to hardware. The latter option provides a consistent programming model for ROS applications, independently of the mapping of ROS nodes to software or hardware.

The remainder of the paper is organized as follows: Section~\ref{sec:BackgroundRelatedWork} provides an overview over ROS and related approaches for integrating hardware accelerators into ROS. Section~\ref{sec:DesignConsiderations} elaborates on different approaches for accelerating ROS applications, before Section~\ref{sec:ReconROS} details {\sc ReconROS} with its architecture and design flow. In Section~\ref{sec:Evaluation}, we present experiments to quantify overheads involved when mapping ROS nodes to hardware and to demonstrate the feasibility and flexibility of {\sc ReconROS}. Finally, Section~\ref{sec:ConclusionFuture Work} concludes the paper and gives an outlook to future work.


